WARP: Word-level Adversarial ReProgramming

Transfer learning from pretrained language models recently became the dominant approach for solving many NLP tasks. A common approach to transfer learning for multiple tasks that maximize parameter sharing trains one or more task-specific layers on top of the language model. In this paper, we present an alternative approach based on adversarial reprogramming, which extends earlier work on automatic prompt generation. Adversarial reprogramming attempts to learn task-specific word embeddings that, when concatenated to the input text, instruct the language model to solve the specified task. Using up to 25K trainable parameters per task, this approach outperforms all existing methods with up to 25M trainable parameters on the public leaderboard of the GLUE benchmark. Our method, initialized with task-specific human-readable prompts, also works in a few-shot setting, outperforming GPT-3 on two SuperGLUE tasks with just 32 training samples.

==> tables/autoprompt_sst.tex <==

\begin{table}[]
\centering
\begin{tabular}{lccr} \hline

\textbf{Approach} &
\textbf{Dev} &
% \textbf{Test} & 
\textbf{\# of parameters} \\
% \hline
% BERT-base       &  $92.7$ &  $93.5$ &  $110\cdot10^6$ \\
% TinyBERT$_6$    &  $93.0$ &  $93.1$ &   $67\cdot10^6$ \\
% TinyBERT$_4$    &  $92.6$ &  $92.6$ &   $15\cdot10^6$ \\
\hline
Fine-tuned      &  $96.4$ &  $335\cdot10^6$ \\
% Adapters        &  $96.3$ &    $3\cdot10^6$ \\
% Single Layer    &  $88.4$ &          $10^6$ \\
Linear Probing  &  $88.4$ &          $2048$ \\
Manual Prompt   &  $85.0$ &             -   \\
AutoPrompt      &  $91.2$ &             -   \\
\hline
WARP\textsubscript{0} & $89.8$ & $2048$ \\
WARP\textsubscript{1} & $93.8$ & $3072$ \\
WARP\textsubscript{2} & $94.3$ & $4096$ \\
WARP\textsubscript{4} & $95.9$ & $6144$ \\
WARP\textsubscript{8} & $95.4$ & $10240$ \\
\hline
WARP\textsubscript{best} & $95.4$ & $22528$ \\

\hline
% WARP$_4^*$ &  95.8   &   96.1   &   6144
% (init with "... Movie was ___  !")
\end{tabular}
\caption{Accuracy on SST-2 development and test sets. The last column shows the number of \textit{trainable} parameters only. All methods use RoBERTa-large if not stated otherwise.
WARP$_K$ corresponds to a prompt consisting of $K$ tokens.
% The subscript next to TinyBERT corresponds to the number of layers in the model. % The prompt for WARP$_4^*$ is initialized with ``... Movie was \_\_\_!''
}
\label{tab:sst}
\end{table}

==> tables/prompts.tex <==
\begin{table}[]
\begin{tabular}{lllllllllllllllllllllll}
Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯ &
  Tomorrow &
  Ale &
  .âĢĵ &
  Ġ*. &
  \textless{}sentence\textgreater{} &
  ĠMUCH &
  irin &
  {[}/ &
  Ġå &
  Ġ(@ &
  \textless{}mask\textgreater{} &
  ĠðŁ &
  ãĤĴ &
  É &
  \textless{}mask\textgreater{} &
  ĠâĶĤ &
  \textless{}sentence\textgreater{} &
  Ġ\textless{}!-- &
  Ġinforming &
  inyl &
  Ġentit &
  dim \\
*. &
  Ġneigh &
  \textless{}mask\textgreater{} &
  Û &
  Ġ\{\{ &
  \textless{}sentence\textgreater{} &
  âĢ¦âĢ¦ &
  \textless{}mask\textgreater{} &
  olitan &
  Ġpronouns &
  \textless{}mask\textgreater{} &
  \textless{}mask\textgreater{} &
  \textless{}mask\textgreater{} &
  @@@@ &
  \textless{}mask\textgreater{} &
  ĠChoi &
  \textless{}mask\textgreater{} &
  \textless{}sentence\textgreater{} &
  $\sim$$\sim$$\sim$ &
  $\sim$$\sim$$\sim$ &
  $\sim$$\sim$$\sim$ &
  $\sim$$\sim$$\sim$ &
  $\sim$$\sim$$\sim$ \\
Ġresembling &
  Ġswarm &
  ĠParamount &
  ĠCalm &
  ĠMembership &
  \textless{}sentence\textgreater{} &
  Ġderive &
  rics &
  \textless{}mask\textgreater{} &
  Ġalias &
  iary &
  \textless{}mask\textgreater{} &
  Ġomnip &
  \textless{}mask\textgreater{} &
  \textless{}mask\textgreater{} &
  \textless{}mask\textgreater{} &
  Ġsham &
  \textless{}sentence\textgreater{} &
  \textless{}mask\textgreater{} &
  Ġforb &
  \textless{}mask\textgreater{} &
  ĠFirefly &
  ĠTHEY \\
Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯ &
  Tomorrow &
  ALE &
  .âĢĵ &
  Ġ*. &
  \textless{}sentence\textgreater{} &
  ĠMUCH &
  irin &
  {[}/ &
  Ġå &
  Ġ(@ &
  \textless{}mask\textgreater{} &
  \_ &
  ãĤĴ &
  femin &
  \textless{}mask\textgreater{} &
  ĠâĶ &
  \textless{}sentence\textgreater{} &
  ãħĭãħĭ &
  Ġinforming &
  \#$#$ &
  Ġentit &
  OOOO \\
choes &
  Ġcharms &
  Ġsorely &
  Ġ"... &
  âĸĳâĸĳ &
  \textless{}sentence\textgreater{} &
  ä &
  afe &
  ¶æ &
  Ġcharred &
  Ġmasked &
  \textless{}mask\textgreater{} &
  ĠFall &
  Ġbabys &
  Ġsmartest &
  íķ &
  ÷ &
  \textless{}sentence\textgreater{} &
  ðĿ &
  forums &
  Ġbio &
  Ġmang &
  Ä± \\
Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯ &
  Tomorrow &
  rison &
  .âĢĵ &
  Ġ*. &
  \textless{}sentence\textgreater{} &
  ĠMUCH &
  irin &
  {[}/ &
  Ġå &
  jay &
  \textless{}mask\textgreater{} &
  ĠðŁ &
  ãĤĴ &
  femin &
  \textless{}mask\textgreater{} &
  .? &
  \textless{}sentence\textgreater{} &
  \_\textgreater{} &
  Ġinforming &
  \#$#$ &
  Ġentit &
  OOOO \\
\textless{}mask\textgreater{} &
  \textless{}mask\textgreater{} &
  \textless{}mask\textgreater{} &
  \textless{}mask\textgreater{} &
  \textless{}mask\textgreater{} &
  \textless{}sentence\textgreater{} &
  \textless{}mask\textgreater{} &
  \textless{}mask\textgreater{} &
  \textless{}mask\textgreater{} &
  \textless{}mask\textgreater{} &
  \textless{}mask\textgreater{} &
  \textless{}mask\textgreater{} &
  \textless{}mask\textgreater{} &
  \textless{}mask\textgreater{} &
  \textless{}mask\textgreater{} &
  \textless{}mask\textgreater{} &
  \textless{}mask\textgreater{} &
  \textless{}sentence\textgreater{} &
  \textless{}mask\textgreater{} &
  \textless{}mask\textgreater{} &
  \textless{}mask\textgreater{} &
  \textless{}mask\textgreater{} &
  \textless{}mask\textgreater{} \\
Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯ &
  Tomorrow &
  Ale &
  .âĢĵ &
  \textless{}mask\textgreater{} &
  \textless{}sentence\textgreater{} &
  ĠKers &
  irin &
  {[}/ &
  Ġå &
  Ġ(@ &
  \textless{}mask\textgreater{} &
  ĠðŁ &
  ÃĥÃĤÃĥÃĤ &
  femin &
  \textless{}mask\textgreater{} &
  ĠâĶĤ &
  \textless{}sentence\textgreater{} &
  Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯Â¯ &
  Ġrepertoire &
  inyl &
  ĠIdea &
  dim
\end{tabular}
\end{table}
